Towards Efficient Design Verification -- Constrained Random Verification using PyUVM

Python, as a multi-paradigm language known for its ease of integration with other languages, has gained significant attention among verification engineers recently. A Python-based verification environment capitalizes on open-source frameworks such as PyUVM providing Python-based UVM 1.2 implementation and PyVSC facilitating constrained randomization and functional coverage. These libraries play a pivotal role in expediting test development and hold promise for reducing setup costs. The goal of this paper is to evaluate the effectiveness of PyUVM verification testbenches across various design IPs, aiming for a comprehensive comparison of their features and performance metrics with the established SystemVerilog-UVM methodology.

==> figures/python_project_ver.tex <==
\begin{tikzpicture}
	\begin{axis}[
		xbar=0pt,
		xmin=0,
		width=10cm,
		height=5cm,
		xmax=90,
		bar width=7pt,
		enlarge x limits={value=0.02,upper},
		legend pos={south east,font=\footnotesize},
		xlabel={Design Projects (\%)},
		symbolic y coords={Other,Cocotb or other methodologies, Stimulus generation,Runtime management},
		ytick=data,
		y tick label style={anchor=east,font=\footnotesize}
		]
		\addplot[fill=black!20,font=\footnotesize] coordinates {(6,Other) (19,Cocotb or other methodologies) (49.6,Stimulus generation) (83.8,Runtime management)};
		\addplot[fill=black!2,,font=\footnotesize] coordinates {(10.3,Other) (26.5,Cocotb or other methodologies) (50,Stimulus generation) (81.6,Runtime management)};
		
		\legend{FPGA,ASIC}
	\end{axis}
\end{tikzpicture}

==> figures/sv_uvm_figure.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
	%uncomment if require: \path (0,769); %set diagram left start at 0, and has height of 769
	
	%Shape: Rectangle [id:dp8711717761049389] 
	\draw  [fill={rgb, 255:red, 128; green, 128; blue, 128 }  ,fill opacity=0.08 ] (100.56,31) -- (560.15,31) -- (560.15,500.22) -- (100.56,500.22) -- cycle ;
	%Shape: Rectangle [id:dp06295001040034864] 
	\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.2 ] (120.56,61.27) -- (539.65,61.27) -- (539.65,351) -- (120.56,351) -- cycle ;
	%Shape: Rectangle [id:dp7498080961585827] 
	\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (141,111) -- (520,111) -- (520,171) -- (141,171) -- cycle ;
	%Shape: Rectangle [id:dp6826541206425283] 
	\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (141,450.5) -- (520,450.5) -- (520,487) -- (141,487) -- cycle ;
	%Shape: Rectangle [id:dp33247566779939897] 
	\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (141,384) -- (520,384) -- (520,420.5) -- (141,420.5) -- cycle ;
	%Shape: Rectangle [id:dp4772471907200009] 
	\draw   (141,205) -- (362,205) -- (362,327.5) -- (141,327.5) -- cycle ;
	%Shape: Rectangle [id:dp2831438189262294] 
	\draw   (402,205) -- (520,205) -- (520,327.5) -- (402,327.5) -- cycle ;
	%Shape: Rectangle [id:dp24226509696882093] 
	\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (153,233.25) -- (246,233.25) -- (246,260.75) -- (153,260.75) -- cycle ;
	%Shape: Rectangle [id:dp4167888790882992] 
	\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (153,289.25) -- (246,289.25) -- (246,316.75) -- (153,316.75) -- cycle ;
	%Shape: Rectangle [id:dp22875501544983545] 
	\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (259,289.25) -- (352,289.25) -- (352,316.75) -- (259,316.75) -- cycle ;
	%Shape: Rectangle [id:dp8745630542503298] 
	\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (414,289.25) -- (507,289.25) -- (507,316.75) -- (414,316.75) -- cycle ;
	%Straight Lines [id:da999193759890673] 
	\draw    (198.5,376) -- (198.5,325.5)(201.5,376) -- (201.5,325.5) ;
	\draw [shift={(200,317.5)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
	\draw [shift={(200,384)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
	%Straight Lines [id:da8639963251476654] 
	\draw    (303.5,384.5) -- (303.5,325.5)(306.5,384.5) -- (306.5,325.5) ;
	\draw [shift={(305,317.5)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
	%Straight Lines [id:da6618561516547166] 
	\draw    (458.5,384.5) -- (458.5,325.5)(461.5,384.5) -- (461.5,325.5) ;
	\draw [shift={(460,317.5)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
	%Straight Lines [id:da3895760716229226] 
	\draw    (201.5,261.5) -- (201.5,281.5)(198.5,261.5) -- (198.5,281.5) ;
	\draw [shift={(200,289.5)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
	%Straight Lines [id:da34395870218669833] 
	\draw    (274.5,288.51) -- (273.57,178.51)(277.5,288.49) -- (276.57,178.49) ;
	\draw [shift={(275,170.5)}, rotate = 449.51] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
	%Straight Lines [id:da1861791374680395] 
	\draw    (430.5,289.51) -- (429.57,179.51)(433.5,289.49) -- (432.57,179.49) ;
	\draw [shift={(431,171.5)}, rotate = 449.51] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
	%Straight Lines [id:da6304352403474731] 
	\draw    (200,421) -- (200,450) ;
	%Straight Lines [id:da3096711245627075] 
	\draw    (305,420) -- (305,451) ;
	%Straight Lines [id:da5703631119510673] 
	\draw    (460,420.5) -- (460,450) ;
	
	% Text Node
	\draw (107,34) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\fontfamily{ptm}\selectfont Test}};
	% Text Node
	\draw (129,68) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\fontfamily{ptm}\selectfont Environment}};
	% Text Node
	\draw (306,210) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\fontfamily{ptm}\selectfont Active }\\{\fontfamily{ptm}\selectfont Agent}};
	% Text Node
	\draw (463,209) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\fontfamily{ptm}\selectfont Passive }\\{\fontfamily{ptm}\selectfont Agent}};
	% Text Node
	\draw (281,294) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\fontfamily{ptm}\selectfont {\small Monitor}}};
	% Text Node
	\draw (435,294) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\fontfamily{ptm}\selectfont {\small Monitor}}};
	% Text Node
	\draw (180,294) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\fontfamily{ptm}\selectfont {\small Driver}}};
	% Text Node
	\draw (170,237) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\fontfamily{ptm}\selectfont {\small Sequencer}}};
	% Text Node
	\draw (297,392) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\fontfamily{ptm}\selectfont Interface}};
	% Text Node
	\draw (246,460) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\fontfamily{ptm}\selectfont Design Under Verification}};
	% Text Node
	\draw (293,132) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\fontfamily{ptm}\selectfont Scoreboard}};
	
	
\end{tikzpicture}


==> src/acronyms.tex <==

	

